Hypothesis Testing the Circuit Hypothesis in LLMs

Large language models (LLMs) demonstrate surprising capabilities, but we do not understand how they are implemented. One hypothesis suggests that these capabilities are primarily executed by small subnetworks within the LLM, known as circuits. But how can we evaluate this hypothesis? In this paper, we formalize a set of criteria that a circuit is hypothesized to meet and develop a suite of hypothesis tests to evaluate how well circuits satisfy them. The criteria focus on the extent to which the LLM's behavior is preserved, the degree of localization of this behavior, and whether the circuit is minimal. We apply these tests to six circuits described in the research literature. We find that synthetic circuits -- circuits that are hard-coded in the model -- align with the idealized properties. Circuits discovered in Transformer models satisfy the criteria to varying degrees. To facilitate future empirical studies of circuits, we created the \textit{circuitry} package, a wrapper around the \textit{TransformerLens} library, which abstracts away lower-level manipulations of hooks and activations. The software is available at \url{https://github.com/blei-lab/circuitry}.

==> preamble/format.tex <==
% ===== fonts

\newif\ifmtpro
\newif\ifsimple
\newif\ifhipster

\mtprotrue
%\simpletrue
%\hipstertrue

% option I: mtpro

\ifmtpro
\usepackage[T1]{fontenc}
\usepackage[full]{textcomp}
\usepackage{newtxtext}
\usepackage{cabin} % sans serif
\usepackage[varqu,varl]{inconsolata} % sans serif typewriter
\usepackage[final,expansion=alltext]{microtype}
\usepackage[english]{babel}

% \usepackage[amssymbols,
%  subscriptcorrection,
%  slantedGreek,
%  nofontinfo,
%  mtpcal,
%  mtpbb]{mtpro2}

\usepackage{bm}
\fi

% option II: simple

\ifsimple
\usepackage[T1]{fontenc}
\usepackage{ccfonts}
\usepackage{amssymb}
\usepackage[bb=mt,cal=mt]{mathalpha}
\fi

% option III: hipster latex

\ifhipster
\usepackage{ccfonts}
\usepackage[T1]{fontenc}
\usepackage{textcomp}
\usepackage[final]{microtype}
\usepackage[english]{babel}

\renewcommand{\familydefault}{lmtt}
\renewcommand{\rmdefault}{lmtt}

\usepackage{amssymb}
% \usepackage[bb=mt,cal=mt]{mathalpha}
\usepackage{mathbbol}
\usepackage{upgreek}

\usepackage{everysel}
\EverySelectfont{% for justification
  \fontdimen2\font=0.4em% interword space
  \fontdimen3\font=0.2em% interword stretch
  \fontdimen4\font=0.1em% interword shrink
  \fontdimen7\font=0.1em% extra space
  \hyphenchar\font=`\-% to allow hyphenation
}
\usepackage{bm}

\fi

% ====== math

\usepackage{amsfonts}
\usepackage{eucal}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{mathtools}

% ===== spacing and text

\usepackage[parfill]{parskip}
\setlength{\parindent}{0pt}
\setlength{\parskip}{2ex plus 0.2ex minus 0.2ex}
\usepackage{afterpage}
\usepackage{setspace} % e.g. \onehalfspacing

% ===== sections and title

\RequirePackage[bf,tiny]{titlesec}

% ===== geometry

\usepackage[
paper  = letterpaper,
left   = 1.25in,
right  = 1.25in,
top    = 1.0in,
bottom = 1.0in,
]{geometry}


%%% Local Variables:
%%% mode: plain-tex
%%% TeX-master: t
%%% End:

==> preamble/preamble.tex <==
% ===== color

\usepackage[usenames,dvipsnames]{xcolor}

% ===== editing

\usepackage{lineno}
\setlength\linenumbersep{5pt}
\renewcommand\linenumberfont{
  \normalfont
  \tiny
  \sffamily
  \color{SkyBlue}}

% ===== nice to dos

% note: pass in "disable" to turn off the to do notes.

\usepackage[colorinlistoftodos,
prependcaption,
textsize=footnotesize,
backgroundcolor=blue!10,
linecolor=black!10,
bordercolor=blue!10]{todonotes}

\newcommand{\db}[1]{\todo[inline]{\textbf{db /} \, \, \, #1}}

% ===== tikz
\usepackage{tikz}
\usetikzlibrary{shapes,decorations,arrows,calc,arrows.meta,fit,positioning}
\tikzset{
    -Latex,auto,node distance =1 cm and 1 cm,semithick,
    state/.style ={ellipse, draw, minimum width = 0.7 cm},
    point/.style = {circle, draw, inner sep=0.04cm,fill,node contents={}},
    bidirected/.style={Latex-Latex,dashed},
    el/.style = {inner sep=2pt, align=left, sloped}
}
\usetikzlibrary{bayesnet}

% ===== figures
\usepackage{graphicx}
\usepackage[labelfont=bf]{caption}
\usepackage[format=hang]{subcaption}

% ===== algorithms

\usepackage[algoruled,ruled,vlined,linesnumbered]{algorithm2e}
\setlength{\algomargin}{1.5em}

% \usepackage{algpseudocode}

% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{algorithmic}
% \usepackage{algorithm}
% ===== listings (for code)

\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\normalsize}

\lstdefinestyle{mystyle}{
    commentstyle=\color{OliveGreen},
    keywordstyle=\color{BurntOrange},
    numberstyle=\tiny\color{black!60},
    stringstyle=\color{darkblue},
    basicstyle=\ttfamily,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=mystyle}

% ===== lists

\usepackage{enumitem}
\renewcommand{\labelitemi}{{\color{black!30}\textbullet}}

% ===== bibliography

% \usepackage{natbib}
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=MidnightBlue}
\hypersetup{urlcolor=MidnightBlue}
\hypersetup{linkcolor=black}

% ===== clever reference

\usepackage[nameinlink]{cleveref}
\creflabelformat{equation}{#1#2#3}
\crefname{equation}{eq.}{eqs.}
\Crefname{equation}{Eq.}{Eqs.}
\Crefname{section}{\S}{\S}

% ===== acronyms and glossaries

\usepackage
[acronym,nowarn,section,nogroupskip,nonumberlist]{glossaries}
\glsdisablehyper{}
\setglossarystyle{long3col}
\setlength\glsdescwidth{0.8\linewidth}
\setlength\glspagelistwidth{0pt}
\makeglossaries

% ===== useful packages

\usepackage{blindtext}
\usepackage{framed}

% ===== tables

\usepackage{booktabs}
\usepackage{multirow}
\usepackage{longtable}
\usepackage{etoolbox,siunitx}
\robustify\bfseries
\sisetup{detect-weight=true, detect-shape=true, detect-mode=true,
  table-format=5.1, table-number-alignment=center}

% ===== other useful commands

\newcommand{\pp}{\noindent \textcolor{lightgray}{\P} \quad}
\newcommand{\qq}{\noindent \textcolor{black}{\textbf{\textsc{q}}} \quad}

\newcommand{\draftdisclaimer}{\textit{Draft of \today: Please do not
    cite or distribute}}

\newcommand{\important}[1]
{
  \vspace{0.1in}
  \begin{shaded}
    \textbf{#1}
  \end{shaded}
}

% ===== title and parhead

\DeclareRobustCommand{\parhead}[1]{\textbf{#1}~}

\newcommand{\mytitle}[2]{
  \begin{center}
    \large \textbf{#1} \\
    \normalsize
    \vspace{0.1in}
    #2 \\
    \vspace{0.25in}
    \today
    \vspace{0.25in}
  \end{center}
}







